Elliptically-Contoured Tensor-variate Distributions with Application to Improved Image Learning

Statistical analysis of tensor-valued data has largely used the tensor-variate normal (TVN) distribution that may be inadequate when data comes from distributions with heavier or lighter tails. We study a general family of elliptically contoured (EC) tensor-variate distributions and derive its characterizations, moments, marginal and conditional distributions, and the EC Wishart distribution. We describe procedures for maximum likelihood estimation from data that are (1) uncorrelated draws from an EC distribution, (2) from a scale mixture of the TVN distribution, and (3) from an underlying but unknown EC distribution, where we extend Tyler's robust estimator. A detailed simulation study highlights the benefits of choosing an EC distribution over the TVN for heavier-tailed data. We develop tensor-variate classification rules using discriminant analysis and EC errors and show that they better predict cats and dogs from images in the Animal Faces-HQ dataset than the TVN-based rules. A novel tensor-on-tensor regression and tensor-variate analysis of variance (TANOVA) framework under EC errors is also demonstrated to better characterize gender, age and ethnic origin than the usual TVN-based TANOVA in the celebrated Labeled Faces of the Wild dataset.

==> sections/MLE.tex <==
\section{Maximum likelihood estimation}\label{sec:MLE}
This section derives MLEs from EC tensor-variate distributed data under four
different scenarios.  We first derive these estimators from
uncorrelated draws that have common and joint %but general (marginal)
EC tensor-variate distributions. This procedure depends on
identifiable MLEs from the TVN distribution, and so we also
describe how to obtain such estimates.
Next, we provide  expectation conditional maximization (ECM)
\citep{dempsterandetal77,mengandrubin93}  and  ECM Either
(ECME) \citep{liuandrubin94} algorithms for maximum likelihood estimation on
IID realizations from a scale TVN mixture distribution, and show how
these estimation algorithms can be used to extend the ToTR framework
of \citep{llosaandmaitra20} to the case where the error distribution
is a scale mixture of TVNs.
 Finally, we derive a robust estimation algorithm for the scale matrices in the
spirit of Tyler's estimation \citep{tyler83,tyler87a,tyler87b} for
unknown EC distributions.



\subsection{Estimation in the TVN model}\label{sec:tensnormalMLE}

Suppose that we independently observe $\mY_1,\mY_2,\dots,\mY_n$ from $\N_{\bbm}(0,\sigma^2\Sigma_1,\Sigma_2,\dots,\Sigma_p)$. The MLEs of the scale matrices $\Sigma_1,\Sigma_2,\dots,\Sigma_p$  are not identifiable since $\Sigma_k \otimes \Sigma_l =
(a\Sigma_k) \otimes (\Sigma_l/a)$ for any scalar $a\neq 0$. Moreover,
the scale matrix estimators have no closed-form solutions, but each $\hSigma_k$ depends on the rest as $\hSigma_k =\sfS_k/(nm_{-k}\sigma^2)$, where
$
\sfS_k  = \sum_{i=1}^n \mY_{i(k)}
\Sigma_{-k}^{-1}\mY_{i(k)}',$ with $\Sigma_{-k}$ as defined in the
paragraph following Definition~\ref{def:ellipcon}.
The existing methodology \citep{dutilleul99,srivastavaandetal08,dutilleul18,rosandetal16,soloveychikandtryshin16}
takes into account the indeterminacy of the estimates by scaling each
$\hSigma_k$ such that the trace, determinant or $(1,1)$th element is
unity. Alternatively, we use the ADJUST procedure of \citet{glanzandcarvalho18} that optimizes the loglikelihood with respect to $\Sigma_k$ under the constraint $\Sigma_k(1,1)=1$ as
$
\hSigma_k = ADJUST(nm_{-k},\sigma^2,\sfS_k).
$
Here $\sigma^2$ is inexpensively estimated to be 
$\hat\sigma^2=\tr(S_k\hSigma_k^{-1})/(nm)$. These form our minor modifications to
the maximum likelihood estimation algorithm of \citet{akdemirandgupta11,hoff11,manceuranddutilleul13,ohlsonandetal13}, but will be used in the following section.

\subsection{Estimation from uncorrelated data with identical
  EC-distributed marginal distributions}\label{sec:uncorrML}
Suppose that we observe realizations $\mY_1,\mY_2,\sdots,\mY_n$ of random
tensors that have the same setting as Theorem \ref{thm:tenswish1}. Our
derivation of MLEs  under the joint EC distributional
assumption of \eqref{eq:jointfull} is then a tensor-variate extension
of Theorem 1 of \citet{andersonandetal86}, and is as follows:
\begin{theorem}\label{mluncorrelated}
Suppose that the density generator $g(\cdot)$ of $\rtY$ is such that 
$
h(d) = 
d^{nm/2}g(d) 
$
has a finite positive maximum $d_g$. Also, let $(\tilde{\sigma}^2,\tilde{\mM},
\tilde\Sigma_1,\tilde\Sigma_2,\dots,\tilde\Sigma_p)$
be the TVN MLEs described in Section \ref{sec:tensnormalMLE}. Then the MLE for $(\sigma^2,\mM,\Sigma_1,\Sigma_2,\dots,\Sigma_p)$ is\newline $(\frac{nm}{d_g}\tilde{\sigma}^2,\tilde{\mM},\tilde\Sigma_1,\tilde\Sigma_2,\dots,\tilde\Sigma_p)$.
\end{theorem}
\begin{proof}
See the Supplementary Material Section \ref{proof:mluncorrelated}.
\end{proof}

It follows that $d_g = mn$ in the TVN case, $d_g = nmb/a$ when $g(\cdot)$ is
of the form \eqref{dengengamma},  $d_g = (mn/s)^{1/s}$ in the power exponential case, and $d_g$ is the solution to 
$
mn/(2d)  = \tanh\left(d/2\right)
$
in the logistic case~\citep{galeaandriquelme00,fangetal90}.
\begin{comment}
In Theorem \ref{mluncorrelated},  for a sample of size $n$ 
conditionally drawn from $\N_{m_1,m_2,\dots,m_p} (\mM_n, \sigma^2
\Sigma_1, \Sigma_2,\dots, \Sigma_p)$, with $\sigma^2$ arising from a
distribution with  positive support, the unconditional joint
distribution of each sample realization is  $\EC_{m_1,\dots,m_p,n} (\mM_n, $ $ \Sigma_1, \dots, \Sigma_p,I_n,\varphi)$, with $\varphi$ determined by the distribution of $\sigma^2$.
This explains why the MLEs for the mean and the
proportionally-constrained $\Sigma_1,\dots,\Sigma_p$ matrices
are the same in both cases, while the estimate of $\sigma^2$ changes
by a proportional constant. When the TVN distribution is fit to a
sample with heavier or lighter tails, then the correction on $\sigma^2$
described in Theorem \ref{mluncorrelated} helps robustify the
estimation by assuming that the data come from a more flexible
EC distribution. 
\end{comment}
\subsection{Estimation from TVN scale mixture realizations}\label{sec:ECtensMLE}

Suppose that we observe $n$ IID realizations $\mY_1,\mY_2,\dots,\mY_n$
from the scale mixture distribution of \eqref{eq:scaletensnorm}. The complete-data loglikelihood is
\begin{equation}\label{eq:completelog}
\ell_c(\boldsymbol{\theta}) = -\dfrac{n}{2} \log|\sigma^2\Sigma| -\dfrac{1}{2\sigma^2}\sum_{i=1}^n z_i D^2_{\Sigma}(\mY_i,\mM) 
%+ \sum_{i=1}^n \log(f_{Z_i}(z_i)).
\end{equation}
where $\boldsymbol{\theta}  
= \left((\vecc\mM)^\top,\boldsymbol{\theta}_{\Sigma}^\top \right)^\top$,
and
$ \boldsymbol{\theta}_{\Sigma}
=
 \big(\sigma^2,(\vecc\Sigma_1)^\top,(\vecc\Sigma_2)^\top\dots,$ $ (\vecc\Sigma_p)^\top\big)^\top.$
 We now use $\ell_c$ to propose an EM algorithm with the following expectation
 (E) and conditional maximization (CM) steps:
\newline
\textbf{E-step:} Here, we obtain the conditional
expectation of \eqref{eq:completelog}, given the  observed data and
evaluated at the $t$th parameter iteration
$\boldsymbol{\theta}^{(t)}$, to get
\begin{equation}\label{eq:expectedcompletelog1}
Q(\boldsymbol{\theta};\boldsymbol{\theta}^{(t)}) = -\dfrac{n}{2} \log|\sigma^2\Sigma|  -\dfrac{1}{2\sigma^2}\sum_{i=1}^n \hat{z}_i^{(t)} D^2_{\Sigma}(\mY_i,\mM),
\end{equation}
where $\hat{z}_i^{(t)}= \mathbb{E}(Z_i|\rtY_i=\mY_i;\boldsymbol{\theta}^{(t)}).$
This conditional expectation depends on the distribution of $Z_i$.
For $Z_i\sim Gamma(a/2,b/2)$, $\rtY_i$ has PDF  given by
\eqref{dengengamma} and  then $\hat{z}_i^{(t)} = {(m+a)}/(D^{2}_{\sigma^{2(t)}\Sigma^{(t)}}(\mY_i,\mM^{(t)})+b).$
\newline
\textbf{CM-steps:} The CM steps maximize 
\eqref{eq:expectedcompletelog1}, but with respect to subsets of parameters. The
first CM step maximizes~\eqref{eq:expectedcompletelog1} with respect to $\mM$ and is obtained by setting to zero
the total differential on $\mM$, that is, 
$\partial Q(\mM) = (\sigma^2)^{-1}\langle \partial \mM, [\![ 
\mS ;
\Sigma_1^{-1},\Sigma_2^{-1},\dots,\Sigma_p^{-1} ]\!] \rangle
 = 0,$ where $\mS =  \sum_{i=1}^n
 \hat{z}_i^{(t)}\mY_i-\mM\sum_{i=1}^n \hat{z}_i^{(t)}.$ The term
 $\partial Q(\mM)=0$ implies that  $\mS =0$, or  
$
\mhM^{(t+1)}  =  (\sum_{i=1}^n \hat{z}_{i}^{(t)} \mY_i) / (\sum_{i=1}^n  \hat{z}_{i}^{(t)}).
$
 Setting  $\mM = \mhM^{(t+1)}$ in  \eqref{eq:expectedcompletelog1}
 profiles out  $\mM$ and again yields \eqref{eq:expectedcompletelog1},
 but with $\mY_{w,i}^{(t)}  = \sqrt{\hat{z}_{i}}^{(t)}(\mY_i -
 \mhM^{(t+1)})$ instead of $\mY_i$.  This profiled loglikelihood is
 identical to the loglikelihood of the TVN model when
 $\mY_{w,i}^{(t)}\sim
 \N_{\bbm}(0,\sigma^2\Sigma_1,\Sigma_2,\dots,\Sigma_p)$, and thus the
 next $(p+1)$ CM steps (corresponding to
 $\sigma^2,\Sigma_1,\Sigma_2,\dots,\Sigma_p$) are obtained similarly
 as for the TVN model of Section \ref{sec:tensnormalMLE}. Specifically, $
\hSigma_k = ADJUST(nm_{-k},\sigma^2,\sfS_k),
$
and $\sigma^2=\tr(S_k\hSigma_k^{-1})/(nm)$. 
\newline
\textbf{EM algorithm:} The ECM algorithm iterates the E- and CM-steps until convergence. We determine convergence based on the relative difference in $||\mM|| + ||\sigma^2\Sigma||,$ where $||\sigma^2\Sigma|| = \sigma^2\prod_{k=1}^p||\Sigma_k||$. The resulting ECM algorithm is summarized in the following steps:
\begin{enumerate}
\item \textbf{Initialization:} Fit the faster TVN model of Section
  \ref{sec:tensnormalMLE} with lax convergence, set $t=0$.
\item 
\textbf{E-Step:} Find $\hat{z}_i^{(t)} := \mathbb{E}(Z_i|\rtY_i=\mY_i;\boldsymbol{\theta}^{(t)})$ $ \forall i=1,2,\dots,n$.
\item 
\textbf{CM-Step 1:} Find $\mhM^{(t+1)}  =  (\sum_{i=1}^n \hat{z}_{i}^{(t)} \mY_i) / (\sum_{i=1}^n  \hat{z}_{i}^{(t)}).$
\item 
\textbf{CM-Step 2:} For each $k=1,2,\dots p$, estimate $\hSigma_k$.
\item
\textbf{CM-Step 3:} estimate $\sigma^2$.
\item
\textbf{Iterate or stop:} Return to the E-step and set $t\gets t+1$, or stop if convergence is met.
\end{enumerate}
\textbf{Alternative EM approach for estimating $\boldsymbol{\sigma^2}$:} 
The above algorithm is an ECM algorithm, since it estimates $\sigma^2$ once for each iteration. A faster alternative is to estimate $\sigma^2$ right after each $\Sigma_k$, making our algorithm an AECM algorithm \citep{mengandvandyk97}. An even faster alternative estimates $\sigma^2$ directly from the loglikelihood 
$\ell(\sigma^2)=
-mn\log(\sigma^2)/2
+\sum_{i=1}^n\log  g (D^{2}_{\Sigma^{(t)}}(\mY_i,\mM^{(t)})/\sigma^2)
$
making the algorithm an ECME algorithm \citep{liuandrubin94}. Our
experiments showed our ECME algorithm to be considerably more
computationally efficient for heavy-tailed EC distributions.


For some cases, such as for the DF parameter in the $t$ distribution, the mixing random variable $Z$ in  \eqref{eq:scaletensnorm} has extra parameters that show up in the last term of the complete loglikelihood \eqref{eq:completelog}, and that may be estimated in  additional
CM steps \citep{liuandrubin95,mcLachlanandkrishnan08}. These extra parameters can also be optimized directly from the loglikelihood as an Either step \citep{liuandrubin94}. For the tensor-variate-$t$ (TV-$t$) distribution with an unknown $\nu$ degree of freedom (the PDF of the TV-$t$ distribution is provided in  \eqref{dengengamma} whenever $a=b=\nu$), we estimate $\nu$ as the solution to
\begin{equation}\label{eq:eithernu}
\begin{split}
0=&1+
\dfrac{1}{n}\sum_{j=1}^n\big[\log z_j^{(k+1)}(\nu)- 
  z_j^{(k+1)}(\nu) \big] 
-%\\-&
\psi(\dfrac{\nu}{2}) + \psi(\dfrac{n+m}{2}) 
+\log(\dfrac{\nu}{2}) - \log(\dfrac{n+m}{2})
\end{split}
\end{equation}
 at each iteration, where
 $
 z_j^{(k+1)}(\nu) = (\nu+m)/(\nu+D^{2}_{\hat\sigma^{2(t)}\hSigma^{(t)}}(\mY_i,\mhM^{(t)})),
 $
 and $\psi$ is the digamma function.
 This is an adaptation of the vector-variate case of \citet{liuandrubin95} to our tensor-variate case.
\subsection{ToTR with scale TVN mixture errors}\label{sec:totr_ec}
 The algorithm proposed in Section \ref{sec:ECtensMLE} can be extended
 to the case where $(\mY_1,\mY_2,\dots,\mY_n)$ are independent
 realizations of the ToTR model, for $i=1,2,\ldots,n$,
\begin{equation}\label{eq:totr}
\mY_i = \langle \mX_i | \mB \rangle+ \mE_i,
\end{equation}
where  $\mX_i$ is the $i$th tensor-variate regression covariate, 
$\mE_i$  the $i$th regression random error following the scale mixture
distribution of \eqref{eq:scaletensnorm} for $\mM = 0$, $\mB$ is the
tensor-variate regression coefficient,  and $\langle . | . \rangle$
denotes the partial contraction as per \eqref{eq:partcontr}. We assume that $\mX_i\in \mathbb{R}^{h_1\times h_2\times \dots \times h_l}$ and $\mY_i \in \mathbb{R}^{m_1\times m_2\times \dots \times m_p}$, which means that $\mB \in\mathbb{R}^{h_1\times h_2\times \dots \times h_l\times m_1\times m_2\times \dots \times m_p }$. 
ToTR was proposed by \citet{hoff14} under TVN errors and outer matrix product (OP) factorization of $\mB$, by \citet{lock17} under {\em canonical polyadic} or CANDECOMP/PARAFAC
(CP) ~\citep{carrollandchang70,harshman70} factorization of $\mB$, by \citep{gahrooeietal21} under the TK factorization, and
by   \citet{liuetal20} under the TT format~\citep{oseledets11} that is the
tensor-ring (TR) format \citep{zhaoetal16a} when one of the TR ranks
is set to 1. The CP, TR, TK and OP factorizations on $\mB$ allow for substantial parameter
reduction without affecting prediction or discrimination ability of the
regression model. For more recent developments in ToTR see \citep{luoandzhang22,raskuttietal19}. The more general case of ToTR can be found under the CP, OP, TR and TK formats and TVN errors in \citet{llosaandmaitra20}, and here we extend these results to the case where the errors follow a scale mixture of TVN distribution.



\subsubsection*{Maximum Likelihood Estimation}
Following the same steps as in Section \ref{sec:ECtensMLE}, the E-step is performed by calculating the expected complete loglikelihood, which can be written as
\begin{equation}\label{eq:expectedcompletelog_totr}
Q(\boldsymbol{\theta};\boldsymbol{\theta}^{(t)}) = -\dfrac{n}{2} \log|\sigma^2\Sigma|  -\dfrac{1}{2\sigma^2}\sum_{i=1}^n D^2_{\Sigma}(\mY_{w,i}^{(t)},\langle \mX_{w,i}^{(t)} | \mB \rangle)
\end{equation}
with $\boldsymbol{\theta} = (\mB,\sigma^2\Sigma)$, and $(\mY_{w,i}^{(t)},\mX_{w,i}^{(t)})=(\sqrt{\hat{z}_i}^{(t)}\mY_i,\sqrt{\hat{z}_i}^{(t)}\mX_i)$ for $\hat{z}_i^{(t)}= \mathbb{E}(Z_i|\rtY_i=\mY_i;\boldsymbol{\theta}^{(t)}).$
For $Z_i\sim Gamma(a/2,b/2)$, we have 
$
\hat{z}_i^{(t)} = {(m+a)}/(D^{2}_{\sigma^{2(t)}\Sigma^{(t)}}(\mY_i,\langle \mX_i|\mB^{(t)} \rangle)+b).
$
 The CM-steps are performed by sequentially optimizing
 \eqref{eq:expectedcompletelog_totr} with respect to the parameter
 factors involved in $\boldsymbol{\theta}$. This equation
 % \eqref{eq:expectedcompletelog_totr}
 is identical to the loglikelihood for the ToTR model under TVN
 errors \citep[see Equation (16) of][]{llosaandmaitra20}, and so the CM-steps
 are performed in one iteration of their block-relaxation algorithm,
 but with $\{(\mY_{w,i}^{(t)},\mX_{w,i}^{(t)}),i=1,2,\dots,n\}$ as the
 responses and covariates. This approach is very general as it works
 for any of the low-rank formats studied in
 \citet{llosaandmaitra20}. The ECM algorithm for maximum likelihood estimation is
 summarized as follows: 
\begin{enumerate}
\item \textbf{Initialization:} Fit the respective ToTR model with TVN errors with a lax convergence. 
\item 
\textbf{E-Step:} Find $\hat{z}_i^{(t)} := \mathbb{E}(Z_i|\rtY_i=\mY_i;\boldsymbol{\theta}^{(t)})$ and $(\mY_{w,i}^{(t)},\mX_{w,i}^{(t)})$ $ \forall i=1,2,\dots,n$.
\item 
\textbf{CM-Step:} Perform one iteration of the respective ToTR algorithm of \citet{llosaandmaitra20}, but with $\{(\mY_{w,i}^{(t)},\mX_{w,i}^{(t)}),i=1,2,\dots,n\}$ as the responses and covariates.
\item
\textbf{Iterate or stop:} Return to the E-step and set $t\gets t+1$, or stop if convergence is met.
\end{enumerate}
Section \ref{sec:classification} later demonstrates that the proposed ToTR
framework with EC errors outperforms ToTR with TVN errors in terms of
classification performance on color bitmap images of cats and dogs
from the AFHQ database.

\subsection{Robust tensor-variate Tyler's estimator}\label{sec:robustmle}
While we proposed several methods for maximum likelihood estimation, they all
require the form of the underlying EC distribution to be known. In this section, we derive constrained MLEs that are robust to the type of EC distribution in the spirit of Tyler's estimator \citep{tyler83,tyler87a,tyler87b,soloveychikandtryshin16}. 
Consider $\rtY_i\sim\EC_{\bbm}(0,\sigma^2\Sigma_1,\Sigma_2,\dots,\Sigma_p,\varphi)$ for $i=1,2,\dots,n$. As described in Section \ref{sec:secproperties}, if we let $\rtZ_i = \rtY_i / ||\rtY_i||$ for all $i=1,2,\dots,n$, then $\vecc(\rtZ_i)\sim\AC_{\bbm}(\Sigma)$, and does not depend on the underlying type of EC distribution. 
Using this result along with the PDF in \eqref{eq:angular_pdf} means
that, regardless of $\varphi$, we can write the loglikelihood for $\Sigma_1,\Sigma_2,\dots,\Sigma_p$ as 
\begin{equation}\label{eq:tyfull}
\ell(\Sigma_1,\Sigma_2,\dots,\Sigma_p) = 
-\dfrac{n}{2} \log\left|\bigotimes_{k=p}^1\Sigma_k\right| 
-\dfrac{m}{2} \sum_{i=1}^n \log D^2_{\Sigma}(\mZ_i,0).
\end{equation}
We now optimize~\eqref{eq:tyfull} using a block-relaxation algorithm \citep{leeuw94} that partitions the parameter space into multiple blocks, and sequentially optimizes each block while fixing the remaining blocks. In this context, each block corresponds to $\Sigma_k$ under the constraint $\Sigma_k(1,1)=1$ for all $k=1,2,\dots,p$, and is derived in the following theorem :
\begin{theorem}\label{thm:tyrobustML}
For a fixed value of $\Sigma_{-k}$ and for $S_{ik} =
\mY_{i(k)}\Sigma_{-k}^{-1}\mY_{i(k)}^\top$, a fixed-point algorithm
for the maximum likelihood estimation of $\Sigma_k$ updates $\Sigma_{k,(t)}$, under the
constraint that $\Sigma_k(1,1) = 1$,  to
\begin{equation}\label{eq:tytensfixed}
\Sigma_{k,(t+1)} = ADJUST\left(n/m_{k},1,\sum_{i=1}^n \dfrac{S_{ik}}{\tr(\Sigma_{k,(t)}^{-1}S_{ik})}\right).
\end{equation}
\end{theorem}
\begin{proof}
See the Supplementary Material Section \ref{proof:tyrobustML}.
\end{proof}
\subsubsection*{ Estimation algorithm}
For each $k$, the fixed-point iteration algorithm of Theorem
\ref{thm:tyrobustML} depends on $\Sigma_{-k}$ only through
$S_{ik}$. Obtaining $S_{ik}$ for all $i=1,2,\dots,n$ and for any
$k=1,2,\dots,p$ has $O(nmm_M)$ computational complexity  (where $m_M=\max\{m_1,m_2,\dots,m_p\}$) while one iteration of \eqref{eq:tytensfixed} is usually considerably cheaper with a complexity of at most $O(m_M^3)$.  Therefore, in most cases we suggest performing $n_L$ iterations of \eqref{eq:tytensfixed} before going from $\Sigma_k$ to $\Sigma_{k+1}$. While all values of $n_L$ will eventually converge, we set $n_L=12$ based on numerical experiments. The final estimation algorithm is  as follows:
\begin{enumerate}
\item \textbf{Initialization:} Fit the TVN model of Section \ref{sec:tensnormalMLE} with lax convergence.
\item For $k=1,2,\dots,p$ 
\begin{enumerate}
\item Obtain $S_{ik}$ from Theorem \ref{thm:tyrobustML} $\forall i=1,\dots,n$
\item Update $\Sigma_{k,(t+1)}$  as per \eqref{eq:tytensfixed} for $n_L$ iterations.
\end{enumerate}
\item
\textbf{Iterate or stop:} Stop if convergence is achieved, or return to Step 2.
\end{enumerate}
\subsubsection*{Robust estimation of the location parameter}\label{subsec:robustM}
When $\mM$ is also unknown, \citet{tyler87a} and
\citet{maronna76} proposed (for the vector-variate case) the  fixed-point iteration algorithm:
$$
\mhM_{(t+1)} = (\sum_{i=1}^n \mX_i/D_{\Sigma}(\mX_i,\mhM_{(t)}))/(\sum_{i=1}^n 1/D_{\Sigma}(\mX_i,\mhM_{(t)}).
$$
\citet{tyler87a} was unable to show the joint existence of $\Sigma$
and $\mM$ due to discontinuities in the objective function, and so we
do not integrate this result into our estimation algorithm. However,
it can be easily integrated to estimate $\mM$ at each iteration and
then used to center the data before estimating
$\Sigma_1,\Sigma_2,\dots,\Sigma_p$. Although to our knowledge, no
theoretical guarantees exist for  this approach even in the
vector-variate case, we have found this algorithm to converge and produce stable estimates  (see Figures \ref{fig:ashoka} and \ref{fig:ashoka_diag}).



\section{Performance Evaluations}
\label{sec:performance}
In this section, we evaluate performance of the maximum likelihood estimation
procedures proposed in Section \ref{sec:MLE} by fitting them to
realizations  from the TVN and from gamma
scale TVN mixture (GSM) distributions. We used the GSM distribution  of
 Section \ref{sec:ECtensMLE}, with PDF as in
\eqref{dengengamma}, $(a,b)=(3,15)$, $i=1,2,\dots,n=10$ and
$(m_1,m_2,m_3,m_4,m_5,m_6) = (7,9,3,23,7,3)$.

  \begin{figure*}[h]
     \centering
     %\figurebox{1pc}{}{}[figures/ashoka.pdf]
     \includegraphics[width = \textwidth]{figures/ashoka.pdf}
     \caption{ \underline{\em Left block}: The Lion
       capital of Ashoka that is the ground truth of the rearranged mean
       tensor $\mM$ of size $7\times 9\times 3\times 23\times 7\times
       3$, and sample realization with increasing variance across
       two EC distributions. \underline{\rm Right
         block:}  Estimated $\mM$ asuming TVN, GSM models
       and Tyler's robust estimators, under TVN and GSM-simulated
       data.  The GSM model-assumed  and Tyler estimators 
       perform similarly as the TVN model-assumed estimators for
       TVN-simulated data, but better than the latter for        GSM-simulated data.} 
     \label{fig:ashoka}
\end{figure*}
% that is the graphic representation
We simulated $\Sigma_k$ (for $k=1,2,\dots,6$) from $\mW_{m_k}(100m_k,I_{m_k})$ or a  Wishart distribution, before constraining
its condition numbers to be at most 50 and scaling each entry by its $(1,1)$th element.  
  The tensor-valued $\mM$ was chosen such that when rearranged in a 3-way
  tensor of size $(7\times9\times 3)\times(23\times 7)\times 3 $, it corresponds to the
  three RGB slices of a $189\times 161$ true color image  of the Lion
  Capital of Ashoka, shown in the leftmost image of Figure \ref{fig:ashoka}. 


We also simulated data for
 $\sigma\in\{2,6,10\}$ and for the TVN case that is a
special case of \eqref{eq:scaletensnorm} when $\Prob(Z_i=1)=1$ for all
$i=1,\dots,n$. Since $\Var(\vecc(\rtY_i)) = 15\sigma^2\Sigma$, 
 we set $\sigma^2$ for TVN-simulated data to be 15 times that of the
 GSM-simulated cases for both sets to have comparable overall
 variability. Figure~\ref{fig:ashoka} (second set of images in the
 left block) displays simulated realizations at each setting: as
 expected, increasing  $\sigma^2$ produces noisier  images.  
  Figure \ref{fig:ashoka} (right block) displays TVN-,
  GSM- and robust-estimated $\mhM$s. For Tyler's robust estimator we used the location  estimation procedure  of Section \ref{subsec:robustM}. 
For all cases, estimation
 performance worsens with increasing $\sigma$. For TVN-simulated data,
 there is little difference in the quality of $\mhM$ obtained by the
 three methods.  % the data is generated from the TVN distribution and estimated by both the TVN and GSM distributions. These two rows show very little difference, indicating the benefit of using the GSM model even when the data originates from a different model. The last two rows show the parameter estimates for $\mM$ when the data is generated from the GSM distribution and estimated by both the TVN and GSM distributions. In this case it is evident that the GSM model results in more accurate parameter estimates, which highlights the sensitivity of the TVN model when the data deviates from normality.
But for heavy-tailed GSM-simulated data, the GSM or robust $\mhM$s
recover $\mM$ better than the TVN-estimated $\mhM$.  

Our illustration in Figure~\ref{fig:ashoka} was only on one
realization for each setting, so we account for simulation variability
in a larger study under a similar framework.
We  generated TVN and GSM data for $\sigma = 2,6,10$ and 100 different
realizations of $(\Sigma_1,\Sigma_2,\dots,\Sigma_6)$, each drawn as before from a Wishart distribution.\begin{figure*}[h]
     \centering
	 \includegraphics[width = \textwidth]{figures/simu1.pdf}
     \caption{ Relative Frobenius norms of differences in parameters
       (generically denoted by $\theta$) for 
       $\sigma\in\{2,6,10\}$, TVN- and GSM-simulated data, and
       estimates obtained under Tyler's robust and GSM model
       assumptions. 
       Each plot is obtained over 100 realizations from
       the  GSM and TVN models with different values of 
     $\Sigma$s, themselves independent
     Wishart realizations. 
     % The magnitude of $\sigma^2$ has little effect on estimating $\Sigma_k$, indicating the estimating models' robustness to increasing variance.
     % Values closer to 1 indicate similar performance of the model to the TVN, while values larger (lower) than 1 indicate better (worse) performance for the estimated model relative to the TVN.
       All points are concentrated around 1 for TVN-simulated data, indicating  that the GSM and Tyler's estimates perform at least as well as the TVN model when the data is TVN-simulated. For the higher dimensional parameters $\mM$ and $\Sigma_4\in\mathbb{R}^{23\times 23}$ and for GSM-simulated data, nearly all points are above 1, indicating that the GSM and Tyler's models outperform the TVN model in this scenario.  For medium-sized parameters $\Sigma_1,\Sigma_2\in \mathbb{R}^{7\times 7}$ and $\Sigma_5\in\mathbb{R}^{9\times 9}$ and for GSM-simulated data, most points are also larger than 1. However, for the smaller $3\times 3$ matrices $\Sigma_3$ and $\Sigma_6$ and for GSM-simulated data, the points are more concentrated at around 1. In conclusion, the GSM and Tyler's models perform at least as well as the TVN model for TVN-simulated data. Morover, the GSM and Tyler's models outperform the TVN model for GSM-simulated data, and their relative performance increase with larger covariance matrices.
    }
     \label{fig:ashoka_diag}
   \end{figure*} 
Figure \ref{fig:ashoka_diag} displays the relative Frobenius norms of the
difference between the true $(\mM,\Sigma_1,\Sigma_2,\dots,\Sigma_6)$ and the estimated $(\hat\mM,\hat\Sigma_1,\hat\Sigma_2,\dots,\hat\Sigma_6)$ parameters, 
 obtained under the GSM, TVN and Tyler models, and for 100 independent samples realized under  GSM and TVN assumptions. 
Specifically, the relative Frobenius normed difference  is $R_d =||\theta - \hat\theta_{TVN}||_2
/||\theta - \hat\theta||_2$, where $\theta$ generically denotes the
parameter being compared, $\hat\theta_{TVN}$ corresponds to the
estimated parameter under the TVN model and $\hat\theta$ denotes the
estimate of the parameter obtained under the assumed GSM or Tyler's
model. Therefore, values larger than unity indicate better performance
of the GSM (or Tyler) estimator over that obtained under  TVN
assumptions. Conversely, values lower than unity indicate worse
performance of GSM (or Tyler) estimates than those obtained under TVN
assumptions.  Our display in Figure~\ref{fig:ashoka_diag} is grouped by parameters of similar
dimensionality, with the first plot displaying results for $\mM$ and $\Sigma_4\in \mathbb{R}^{23\times 23}$, the second one for $\Sigma_1,\Sigma_5 \in \mathbb{R}^{7\times 7}$ and $\Sigma_2\in \mathbb{R}^{9\times 9}$, and the last one for displaying values of the $3\times 3$ matrices $\Sigma_3$ and $\Sigma_6$.
%The scalar variance $\sigma^2$ only marginally affects the performance of $\hat\Sigma_1,\hat\Sigma_2,\dots,\hat\Sigma_6$, illustrating the robustness of the estimating models to increasing values of $\sigma^2$. This is not the case for $\mhM$, whose estimation ability degrades with increasing $\sigma$. 
For TVN-simulated data,  there is not much to choose from betwen the
TVN-assumed estimates and those obtained using  GSM or Tyler
estimators. 
 On the other hand, for GSM-simulated data and the higher dimensional
 parameters $\mM$ and $\Sigma_4$, the  robust GSM and Tyler models
 outperform the TVN model, since nearly all values exceed unity. The
 performance of the TVN model is still worse for
 $\Sigma_1,\Sigma_2,\Sigma_5$ when compared to the GSM and Tyler
 models, since $R_d$ is then mostly above 1. However, for smaller
 $3\times 3$ covariance matrices ($\Sigma_3$ and $\Sigma_6$), the TVN
 model performs more like the GSM and Tyler models. In conclusion, the
 GSM and Tyler fits perform similarly to the TVN model for
 TVN-simulated data. Morover, the GSM and Tyler models outperform the TVN model when the data are GSM-simulated, and their performance relative to the TVN increase with larger covariance matrices.
Our simulation experiment shows the importance of considering an EC
distribution that is more general than the TVN when the tails of the
data are heavier. It also shows the benefit of using Tyler's robust
estimator even when the exact EC distribution is unknown.





==> sections/theory.tex <==
\section{Definitions and Characterizations}\label{sec:ecsec}
\subsection{Background and preliminaries}
\label{sec:prelim}
We define a {\em tensor} as a multi-dimensional array of numbers. This
article uses $\mX$, $\sfX$ and  $X$ to denote deterministic tensors, matrices and
vectors, with bold-faced fonts for their random counterparts ({\em
  e.g.}, $\rtX$, $\rmX$ and $\rvX$ denote random tensors, matrices and vectors). Further, we assume that  $\mX \in \mathbb{R}^{\times_{k=1}^p m_k}$  has $(i_1,i_2\sdots,i_p)$th element written
as $\mX(i_1,i_2,\sdots,i_p)$. 
Tensor reshapings \citep{koldaandbader09} allow us to modify the
structure of a tensor while preserving its elements. We can reshape
$\mX$ into a  $(m_{k})\times(\prod_{i=1,i\neq k}^p m_{i})$-matrix
$\mX_{(k)}$ using its $k$th mode matricization.
The matrix $\mX$ can also be reshaped, by means of its $k$th
canonical matricization, into 
a $(\prod_{i=1}^km_{i})\times(\prod_{i=k+1}^pm_{i})$ matrix
$\mX_{<k>}$, and into a vector $\vecc(\mX)$ of  
$\prod_{i=1}^pm_{i}$ elements using vectorization -- see
\eqref{defvec}, \eqref{kmode} and \eqref{canonical} in
Section~\ref{app:tensdef} for formal definitions. 


The $k$th mode product between $\mX$ and the $n_k\times m_{k}$ matrix
$\sfA_k$ multiplies $\sfA_k$ to the $k$th mode of $\mX$, resulting in
the tensor  $\mX\times_k \sfA_k\in\mathbb{R}^{m_1\times\sdots\times m_{k-1}\times n_k\times m_{k+1}\times\sdots\times m_p}$. 
%that has the same dimensionality as$\mX$ in all modes, except for the $k$th one, where it has size $n_k$.
Applying the $k$th mode product with respect to $\sfA_k$ to every mode of
$\mX$ results in the Tucker (TK) product $[\![\mX;\sfA_1,\sdots,\sfA_p]\!]\in\mathbb{R}^{\times_{k=1}^pn_k}$ \citep{kolda06}. 
%It follows that $\vecc[\![\mX;\sfA_1,\sdots,\sfA_p]\!]=(\bigotimes_{k=p}^1 \sfA_k)vecc(\mX),$where $\otimes$ denotes Kronecker product.
The inner product between two equal-sized tensors $\mX$ and $\mY$ is
defined as $(\vecc\mX)^\top(\vecc\mY)$ and denoted as $\langle\mX,\mY\rangle$. 
 If $\mB$ is a $(p+q)$-way tensor of size $m_1\times m_2\times \ldots \times m_p\times h_1\times h_2\times \ldots \times h_q$, then the partial contraction \citep{llosaandmaitra20} between $\mB$ and $\mX$ (denoted as $\langle \mX|\mB\rangle$) is a $q$-way tensor of size $h_1\times h_2\times \ldots \times h_q$ with 
\begin{equation}\label{eq:partcontr}
\begin{split}
\langle \mX|\mB\rangle(j_1,\dots,j_q)
=%\\=
&\sum_{i_1=1}^{m_1}\ldots \sum_{i_p=1}^{m_p}\mX(i_1, \ldots ,i_p)\mB(i_1, \ldots ,i_p,j_1, \ldots ,j_p).
\end{split}
\end{equation}
We refer to Section \ref{app:tensdef} for the reshaping and product definitions encountered in this section.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



A random tensor $\rtX$ is a tensor whose vectorized form $\vecc(\rtX)$ is a
random vector. 
% The stochastic properties of $\rtX$ and $\vecc(\rtX)$ are identical since both entities have the same elements. 
In many cases $\Var\{\vecc(\rtX)\}=\sigma^2 \otimes_{k=p}^1\Sigma_k$ for
$\Sigma_k\in\mathbb{R}^{m_k\times m_k}$, and the squared Mahalanobis
distance (with respect to the scale matrices $\sigma^2\Sigma_1,\sdots,\Sigma_p$)  of $\rtX$ from its mean $\mbE(\rtX) = \mM$ is 
\begin{equation}\label{eq:mahlanobis}
D^2_{\sigma^2\Sigma}(\rtX,\mM)=
\dfrac{1}{\sigma^2}
\langle
\rtX - \mM
,
[\![\rtX- \mM;\Sigma_1^{-1},\sdots,\Sigma_p^{-1}]\!]
\rangle.
\end{equation} 


A random vector $\bX$ has a vector-valued \textit{spherical}
distribution if its distribution is invariant to rotations: that is, for every $\Gamma\in O(h)= \{H \in 
\mbR^{h\times h} :HH^\top=I_h\}$, we have 
$\bX\overset{d}{=}\Gamma\bX$, or equivalently $\mL(\bX)=\mL(\Gamma\bX)$,
with $\overset{d}{=}$ meaning distributional equality and $\mL(\bX)$ meaning the law of $\bX$.
 This notion of sphericity can be extended to a random matrix $\rmX$
 if it is invariant to rotations of its rows or/and columns
 %, or if $\vecc(\rmX)$ follows a vector-valued spherical distribution
 \citep{fangandchen84}. 	
 %Similarly, spherically-distributed random tensors can be defined in multiple  ways.
In this article, we say that a random tensor $\rtX \in \mathbb{R}^{\times_{k=1}^p m_k}$ follows a tensor-valued spherical distribution if $\vecc(\rtX)$ follows a vector-valued spherical distribution. Thus
$
\vecc(\rtX)\overset{d}{=} \Gamma\vecc(\rtX)
$
 for any $\Gamma\in O(\prod_{k=1}^ph_k)$, meaning that 
 %the characteristic function (CF), $\psi_{\rtX}(\mZ)$, of  is an invariant function
the distribution of  $\rtX$ is invariant
  under the group of transformations $\mathscr{G} =
 \{\varrho_\Gamma:\Gamma \in O(\prod_{k=1}^ph_k)\}$, where
 $\varrho_\Gamma (\rtX) = \Gamma\vecc(\rtX)$ is the matrix product of
 $\vecc(\rtX)$ with
 the orthogonal matrix $\Gamma$. Since $\langle \rtX,\rtX\rangle$ is
 maximally invariant under $\mathscr{G}$ \citep[cf. Example 2.11 of][]{eaton89}, it follows
 that the probability density function (PDF) $f(\cdot)$ and
 characteristic function (CF) $\psi(\cdot)$  are of the form
\begin{equation}\label{spher:cf1}
\psi_{\rtX}(\mZ) = \varphi(\langle \mZ,\mZ\rangle),\quad
f_{\rtX}(\mX) = g(\langle\mX,\mX\rangle)
\end{equation}
for some functions $\varphi$ and $g$ called the characteristic
generator (CG) and probability density generator of $\rtX$.
We write $\rtX \sim \Sph_{h_1,\sdots,h_p}(\varphi)$ if $\rtX$ has
the CF in \eqref{spher:cf1}. We define EC-distributed random tensors
from spherical distributions through the TK product. In the following,
we will define EC distributions that are nonsingular, and have positive definite scale matrices.
\begin{definition}\label{def:ellipcon}
Suppose that $\rtX\sim \Sph_{h_1,\sdots,h_p}(\varphi)$, $\mM \in \mathbb{R}^{\times_{k=1}^pm_k}$, and $\sfQ_k\in \mathbb{R}^{m_{k} \times h_k}$ are matrices such that $\sfQ_k \sfQ_k^\top = \Sigma_k$ is positive definite for all $k = 1,\sdots,p$. Then if 
\begin{equation}\label{eq:defscale}
\rtY \overset{d}{=} \mM+[\![\rtX ; \sfQ_1,\sdots,\sfQ_p ]\!],
\end{equation}
we say that $\rtY$ has an EC distribution with mean $\mM$, scale matrices $\Sigma_1,\Sigma_2,\sdots,\Sigma_p$, and CG $\varphi$, written as $\rtY \sim \EC_{\bbm}(\mM,\Sigma_1,\Sigma_2,\sdots,\Sigma_p,\varphi),$ where $\bbm=(m_1,m_2,\sdots,m_p)^\top$.
\end{definition}
For $\varphi(x) = \exp(-x/2)$% in Definition \ref{def:ellipcon}
,  $\rtY$ follows the TVN distribution $\N_{\bbm}(\mM,\Sigma_1,\sdots,\Sigma_p)$.
We will use
$\bbm\!=\!(m_1,\sdots,m_p),
m=\prod_{i=1}^p m_{i}, 
m_{-k}\!=\!\frac{m}{m_k},
\Sigma \!=\! \otimes_{i=p}^1 \Sigma_i,
\Sigma_{-k}\!=\!\otimes_{i=p,i\neq k}^1 \Sigma_i.
$
%We now characterize an important subfamily of tensor-variate EC  distributions.

%\subsection{Scale Mixture family of TVN distributions}\label{sec:scalemixt}
Scale mixtures of TVN are an important sub-family of EC distributions, and are defined as 
\begin{equation}\label{eq:scaletensnorm}
\mL(\rtY|(Z = z)) =  \N_{\bbm}
(\mM,z^{-1}\Sigma_1,\Sigma_2,\sdots,\Sigma_p)
\end{equation}
for some non-negative random variable $Z$. This distribution is the tensor-variate extension~\citep{arashi17} of
the vector-variate case studied in
\citet{andrewsandmallows74,chu73,yao73} and the matrix-valued case
investigated in \citet{guptaandnagar99,guptaandvarga95}. 
A commonly-used mixing distribution in  \eqref{eq:scaletensnorm}, for the vector-variate case, uses
$Z\sim Gamma(a/2,b/2)$: doing so in the tensor-variate case yields the PDF
\begin{equation}\label{dengengamma}
f_{\rtY}(\mY) = \Big|\pi b\bigotimes_{k=p}^1\Sigma_k\Big|^{-\frac{1}{2}} 
\dfrac{\Gamma((m+a)/2)}{\Gamma(a/2)}
\Big(1+\dfrac{D^2_{\Sigma}(\mY,\mM)}{b}\Big) ^{-\frac{m+a}{2}}
\end{equation}
that corresponds to the TV-$t$ distribution with
$\nu$ degrees of freedom (DF) when $a=b=\nu$, the tensor-variate Cauchy
distribution when additionally $\nu=1$, and 
a tensor-variate Pearson Type VII distribution \citep[cf. page
450,][]{pearson1916}  with parameter $q$ when $a=m$ and $b=q$. We now
derive some useful properties of the EC tensor-variate distribution.

 
 


%\section{Properties of the EC Family of Distributions}
\subsection{Characterizing the EC family of tensor-variate distributions}\label{sec:secproperties}
 Defining EC distributions in terms of
 \eqref{eq:defscale} allows us to extend results from the
 spherical family of distributions to its EC counterpart. For
 instance, from  \eqref{spher:cf1} and \eqref{eq:defscale}, we can write the CF of $\rtY$ in terms of its CG $\varphi$ as
\begin{equation}\label{ellipt:cf1}
\psi_{\rtY}(\mZ) 
=
% \exp(\I\langle \mZ , \mM\rangle)\psi_{\rtX}( [\![\mZ ; \sfQ_1^\top,\sfQ_2,\sdots,\sfQ_p^\top ]\!])=
\exp(\I\langle \mZ , \mM\rangle)\varphi(\langle \mZ , [\![\mZ ; \Sigma_1,\Sigma_2,\sdots,\Sigma_p ]\!]\rangle).
\end{equation}
Similarly, if $\rtX\sim \Sph_{h_1,h_2, \sdots,h_p}(\varphi)$ has the PDF in \eqref{spher:cf1}, then the transformation induced in \eqref{eq:defscale} has Jacobian determinant $|\bigotimes_{k=p}^1\Sigma_k|^{-1/2}$, so the PDF of $\rtY$ is
\begin{equation}\label{ellipt:PDF1}
f_{\rtY}(\mY) = \Big|\bigotimes_{k=p}^1\Sigma_k\Big|^{-1/2} g ( D^2_{\Sigma}(\mY,\mM)),
\end{equation}
where $D^2(\cdot)$ is the squared Mahalanobis distance of \eqref{eq:mahlanobis}. Table~\ref{table:density_generators} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%  TABLE BEGIN  %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[b]
\centering
  \caption{Some common EC distributions, defined using 
    \eqref{ellipt:PDF1} with their  corresponding probability 
    density     generators $g(\dot)$, given upto their constant of proportionality.}
\begin{tabular}{ c | c | c }
    \hline
  Distribution & Additional  & $g(x)$ \\ 
     &  parameters &  \\  \hline 
      Normal  & -- &$\exp(-x/2)$\\
   Student's-$t$  & $q>0$  & $(1+q^{-1}x)^{-(q+m)/2}$\\
   Pearson Type VII  & $q>0$  & $(1+x/q)^{-m}$\\
   Kotz Type  & $q>0$  & $x^{m-1}\exp(-qx)$\\
   Logistic  & -- & $\exp(-x)/(1+\exp(-x))^2$\\
   Power exponential  & $q>0$& $\exp(-x^q/2)$\\  \hline 
     \end{tabular}
\label{table:density_generators}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%  TABLE END  %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
defines some EC distributions by specifying the density generator
function $g(\cdot)$  \citep[see][for additional specifications]{arashiandtabatabaey10,galeaandriquelme00}.

The following theorem allows us to express EC tensor-variate distributions in terms of vector-variate EC distributions that have
been studied extensively in the literature.
\begin{theorem}\label{thm:reshap_EC}
  With the reshapings of \eqref{defvec}, \eqref{kmode} and
  \eqref{canonical}, and for all $k=1,2,\sdots,p$, the following
  statements are equivalent, with $n_k = \prod_{i=1}^k m_{i}$:
\begin{enumerate}
\item \label{reshap:par1} $\rtY \sim \EC_{\bbm}(\mM,\Sigma_1,\Sigma_2,\sdots,\Sigma_p,\varphi)$.
\item \label{reshap:par2}
$
\rtY_{(k)} \sim \EC_{m_{k},m_{-k}} ( \mM_{(k)}, \Sigma_k,  \Sigma_{-k} ,\varphi)$
\item \label{reshap:par3}
$
\rtY_{<k>} \sim \EC_{n_k,m/n_k} ( \mM_{<k>},  \bigotimes_{i=k}^1 \Sigma_i, \bigotimes_{i=p}^{k+1} \Sigma_i ,\varphi)$.
\item \label{reshap:par4} $\vecc(\rtY) \sim \EC_{m} ( \vecc(\mM),  \Sigma ,\varphi)$.
\end{enumerate}
\end{theorem}
\begin{proof}
See the Supplementary Material Section \ref{proof:reshap_EC}.
\end{proof}
%\subsection{Stochastic Representation}\label{sec:stochrep}
Spherical distributions receive their name from the observation that if  $\rtX \sim \Sph_{h_1,h_2,\hdots,h_p}(\varphi)$, then $\rtX = R\rtU,$ where the magnitude $R=||\rtX||$ is independent from $\rtU$
and $\vecc(\rtU)$ is uniformly distributed in the shell of a unit sphere of dimension $\prod_{k=1}^ph_k$ \citep{cambanisetal81,schoenberg38,khokhlov06}. 
Based on the CF in \eqref{spher:cf1} and the independence of $R$ and $\rtU$ , we have that
$
\psi_{\rtX}(\mZ) 
= 
\mbE\{\psi_{\rtU}(R\mZ)\}, 
$
and since $\rtU$ is also spherically distributed, the CG of $\rtX$ can
be written, in terms of the CG of $\rtU$, as
\begin{equation}\label{spher:stocharacgen}
\varphi(u) =\mbE\{\varphi_{\rtU}(R^2u)\}.
\end{equation}
The distribution of $R$ determines the distribution of $\rtX$. For instance, if $R^2\sim\chi^2_h$, where $h=\prod_{k=1}^ph_k$, then 
 $\varphi(u) =
 \exp(-u/2)$ and $\rtX$ follows a TVN distribution.
Further, if
$\rtY\sim\EC_{\bbm}(0,\sigma^2\Sigma_1,\sdots,\Sigma_p,\varphi)$ as in equation \eqref{eq:defscale} and
$\rtX = R\rtU$ as above,
 then $\rtZ
= \rtY/ ||\rtY||$ does not depend on $R$, meaning that the
distribution of $\rtZ$ does not depend on the original
EC distribution of $\rtY$. The distribution of $\rvZ=\vecc(\rtZ)$  is called
the \textit{elliptical angular distribution}
\citep{mardia72,watson83}, and is denoted as $\rvZ\sim\AC_m(\Sigma)$, with PDF 
\begin{equation}\label{eq:angular_pdf}
f_{\rvZ}(\bz) = \frac{\Gamma(m/2)}{2\pi^{m/2}}|\Sigma|^{-1/2}(\bz^\top\Sigma^{-1}\bz)^{-m/2}.
\end{equation}
The above PDF does not depend on $\sigma^2$. In Section
\ref{sec:robustmle}, we derive a robust tensor-variate Tyler
estimator that exploits the fact that $\rtZ$ is the same for any
EC distribution. 

\subsection{Marginal and conditional distributions}
Our next theorem shows that the TK product of an EC distributed
random tensor is also EC distributed. 
\begin{theorem}\label{ellipt:distform} 
Let $\rtY\! \sim\!  \EC_{\bbm}(
\mM,\Sigma_1,\sdots, \Sigma_p, \varphi)$ and $\sfA_k \in \mathbb{R}^{n_k\times m_{k}}$  $\forall k=1,\sdots,p$. Then 
\begin{equation*}
\begin{split}
[\![\rtY; \sfA_1,\sdots,\sfA_p ]\!] \sim \EC_{[n_1 , \sdots , n_p]}&( [\![\mM; \sfA_1,\sdots,\sfA_p ]\!],\sfA_1\Sigma_1\sfA_1^\top,\sdots, \sfA_p\Sigma_p\sfA_p^\top,\varphi).
\end{split}
\end{equation*}
\end{theorem}
\begin{proof}  
See the Supplementary Material Section \ref{proof:ellipt:distform}.
\end{proof}
As a corollary, the marginal distributions follow from Theorem \ref{ellipt:distform} by choosing $\sfA_1,\sdots,\sfA_p$ appropriately, as described in detail in Section \ref{sec:marginals}. 
We now extend the vector-variate result of \citet{cambanisetal81} to derive conditional distributions in the tensor-variate setting.
\begin{theorem}\label{ellipt:conditional}
Suppose that $\rtY \sim \EC_{\bbm}(\mM,\Sigma_1,\sdots,\Sigma_p
,\varphi)$, where $m_p = n_1 + n_2>1$ for some $n_1, n_2 \in
\mathbb{N}$, and $\Sigma_p$ is a block matrix with $(i,j)$th block $\Sigma_{ij} \in \mathbb{R}^{n_i\times n_j}$.
Partition $\rtY$ and $\mM$ over the $pth$ mode with 
$\rtY_1,\mM_1 \in \mathbb{R}^{m_1\times m_2\times\hdots\times m_{p-1}\times
  n_1}$ and $\rtY_2,\mM_2 \in \mathbb{R}^{m_1\times m_2\times \hdots\times
  m_{p-1}\times n_2}$. Then 
\begin{equation}\label{eq:condres}
\begin{split}
\rtY_1|(\rtY_2 = \mY_2)\sim \EC_{[m_1,\sdots,m_{p-1},n_1]}
\Big(
\mM_{\{1\}|\{2\}}
,
\Sigma_1,\sdots,\Sigma_{p-1},
%\\&
\Sigma_{p,\{11\}|\bullet}
,\varphi_{q(\mY_2)}
\Big),
\end{split}
\end{equation}
where
$\mM_{\{1\}|\{2\}} = \mM_1 + (\mY_2 - \mM_2)\times_p(\Sigma_{p,12}\Sigma_{p,22}^{-1})$ 
, 
$\Sigma_{p,\{11\}|\bullet} = \Sigma_{p,11}-\Sigma_{p,12}\Sigma_{p,22}^{-1}\Sigma_{p,21}$
,
$\varphi_{q(\mY_2)}(u) =\mbE\{R^2_{q(\rtY_2)}\varphi_{\rtU}(u)|\rtY_2 = \mY_2\}$,
$
R^2_{q(\rtY_2)} \!=\! D^2_{\Sigma_{\bullet}}(\rtY_1,\mM_1),
$
and
$
\Sigma_{\bullet} \!=\! \Sigma_{p,\{11\}|\bullet}\otimes \Sigma_{-1}.
$
\end{theorem}
\begin{proof}
See the Supplementary Material Section \ref{proof:ellipt:conditional}.
\end{proof}
The CG  $\varphi_q(\mY_2)$ in  \eqref{eq:condres} is a conditional moment, just like in the more general case of \eqref{spher:stocharacgen}. Although Theorem \ref{ellipt:conditional} applies only for the conditional distribution that results from partitioning the last mode of the random tensor, we can find conditional distributions of any subtensor by applying Theorem \ref{ellipt:conditional} multiple times, as demonstrated in Section \ref{supp:condsupp}. 


\subsection{Moments}

  The moments of EC tensor-variate distributions are found by
  differentiating \eqref{ellipt:cf1}. We provide the first four
  moments in Theorem \ref{expectelement} and then use
  them in Theorem \ref{thm:moments_ec} to find moments of other special forms. %All the proofs of this section are found in the Appendix section \ref{app:proofmoments}.
\begin{theorem}\label{expectelement} 
Suppose $\rtY \sim  \EC_{\bbm}( \mM,\Sigma_1,\Sigma_2,\sdots,
\Sigma_p,\varphi)$, and let $\bbi=(i_1,\sdots, i_p)^\top$,
$\bj=(j_1,\sdots,j_p)^\top$, $\bk=(k_1,\sdots,k_p)^\top$ and $\bl=(l_1,\sdots,l_p)^\top$ be sets of indices such that $i_q,j_q,k_q,l_q\in \{1,\sdots,m_q\}$ for $q =1,\sdots,p$. Further, denote $\rtY(i_1,\sdots, i_p)=Y_{\bbi} $, $\mM(i_1,\sdots, i_p)=m_{\bbi}$ and $\sigma_{\bbi\bj} = \prod_{q=1}^p \Sigma_q(i_q,j_q)$. Then
\begin{enumerate}
\item \label{expectelement:1} $\mbE(Y_{\bbi}) = m_{\bbi}$.
\item  \label{expectelement:2}
$\mbE(Y_{\bbi}Y_{\bj}) 
= m_{\bbi}m_{\bj}-2 \varphi'(0)\sigma_{\bbi\bj}$.
\item \label{expectelement:3} $\mbE(Y_{\bbi}Y_{\bj}Y_{\bk}) 
\hspace*{-.1cm}=\hspace*{-.1cm}
 m_{\bbi}m_{\bj}m_{\bk}
 \hspace*{-.1cm}-\hspace*{-.1cm}
 2\varphi'(0)(
m_{\bbi}\sigma_{\bk\bj}
\hspace*{-.1cm}+\hspace*{-.1cm}
m_{\bj} \sigma_{\bbi\bk}
\hspace*{-.1cm}+\hspace*{-.1cm}
m_{\bk}\sigma_{\bbi\bj}
).
$
\item \label{expectelement:4} $\mbE(Y_{\bbi}Y_{\bj}Y_{\bk}Y_{\bl}) = m_{\bbi}m_{\bj}m_{\bk}m_{\bl}
+ 4 \varphi''(0)\Big(\sigma_{\bk\bl}\sigma_{\bj\bbi}
+\sigma_{\bj\bl}\sigma_{\bbi\bk}
+\sigma_{\bbi\bl}\sigma_{\bj\bk}\Big)-2 \varphi'(0)\Big(m_{\bl}m_{\bk}\sigma_{\bbi\bj}
+m_{\bj}m_{\bl}\sigma_{\bbi\bk}
+m_{\bj}m_{\bk}\sigma_{\bbi\bl}
+m_{\bbi}m_{\bl}\sigma_{\bj\bk}
+m_{\bbi}m_{\bk}\sigma_{\bj\bl}
+m_{\bbi}m_{\bj}\sigma_{\bk\bl}\Big).
$
\end{enumerate}
Here, the $k$th statement of the theorem requires $\varphi^{(k)}(0)<\infty$, for $k=1,2,3,4$.
\end{theorem}
\begin{proof}
See  the Supplementary Material Section \ref{app:proofexpectelement}.
\end{proof}
Theorem \ref{ellipt:distform} allows us to derive many different
moments. We derive some of them now.
\begin{theorem}\label{thm:moments_ec}
Let $\rtY \sim \EC_{\bbm}(\mM,\Sigma_1,\Sigma_2,\hdots,\Sigma_p,\varphi)$, where $\varphi''(0)\!<\!\infty$. 
Further, let $\sfA_k$ and $\sfB_k$ be $n_k\times m_k$ and $h_k\times
m_k$ matrices for $k=1,2,\hdots,p$, and define $D^2_A(\mX) = \langle
\mX,[\![\mX;\sfA_1,\sfA_2,\sdots,\sfA_p]\!]\rangle$ whenever each
$A_k$ is a square matrix. Then,
\begin{enumerate}
\item \label{par51} $\mbE(\rtY) = \mM$.
\item \label{par52}
$
\Var\{\vecc(\rtY)\} = -2\varphi'(0)\bigotimes\limits_{k=p}^1 \Sigma_k.
$
\item \label{par54} If $n_k=m_k$ for all $k=1,2,\hdots,p$, then 

$
\mbE\left\{D^2_A(\rtY)\right\} = D^2_A(\mM) -2\varphi'(0)\prod\limits_{k=1}^p \tr(\Sigma_k\sfA_k^\top).
$
\item\label{par55} If $\mV$ is of size $n_1\times n_2\times\hdots\times n_p$, then 
%  \begin{equation*}
%    \begin{split}

$\mbE(\langle \mV,[\![\rtY;\sfA_1,\hdots,\sfA_p]\!]\rangle\rtY) 
=\langle \mV,[\![\mM;\sfA_1,\hdots,\sfA_p]\!]\rangle\mM
 -
2\varphi'(0)[\![\mV;\Sigma_1 \sfA_1^\top,\hdots,\Sigma_p
\sfA_p^\top]\!].
$%\end{split}
%end{equation*}
\item\label{par56} If $n_k=m_k$ for all $k=1,2,\hdots,p$, then
%\begin{equation*}
%\begin{split}
%\mbE\big(D^2_A(\rtY)\rtY\big) = &D^2_A(\mM)\mM

$ -2\varphi'(0)\Big[\prod\limits_{k=1}^p \tr(\Sigma_k\sfA_k^\top)\mM 
 +[\![\mM;\Sigma_1 \sfA_1,\hdots,\Sigma_p \sfA_p]\!] 
%   \\&
   	+
 [\![\mM;\Sigma_1 \sfA_1^\top,\hdots,\Sigma_p \sf A_p^\top]\!]\Big].
$
%\end{split}
%\end{equation*} 
\item \label{par57} If $\mM=0$, $\varphi^{(4)}(0)<\infty$ and $n_k=h_k = m_k$ for all $k=1,\hdots,p$, then 

$\mbE\big
  \{
D^2_A(\rtY)D^2_B(\rtY)
\big\} \!=\!
%&
 4\varphi''(0)\Big[
\prod\limits_{k=1}^p \left\{ \tr(\sfA_k\Sigma_k)\tr(\sfB_k\Sigma_k) \right\}
+
\prod\limits_{k=1}^p \tr(\sfA_k\Sigma_k\sfB_k^\top\Sigma_k) 
%\\&
\!+\!
\prod\limits_{k=1}^p \tr(\sfA_k\Sigma_k\sfB_k\Sigma_k) 
\Big].
$%\end{split}
%\end{equation*}
\end{enumerate}
\end{theorem}
\begin{proof}
See the Supplementary Material Section \ref{proof.b2}.
\end{proof}
From Parts~\ref{par54} and \ref{par57} of Theorem
\ref{thm:moments_ec}, we see that for $\rtY$ specified as in Definition \ref{def:ellipcon},  $\mathbb{E}\{ D^2_{\Sigma}(\rtY,\mM)\}= -2\varphi'(0)\times m
$, and
$
\mathbb{V}ar\{ D^2_{\Sigma}(\rtY,\mM)\}=4\times [\varphi''(0)\times(m^2 + 2m) - (\varphi'(0)\times m)^2]. 
$


\subsection{The EC tensor-variate Wishart distribution} The Wishart
distribution~\citep{wishart28} plays an important role in multivariate
statistics in inference on sample dispersion
matrices \citep{johnsonandwichern08}.  The matrix-variate EC Wishart
distribution was proposed
in~\citet{caroetal14,diazandgutierrez11,sutradharandali89} as per 
\begin{definition}\label{def:matwish}
A matrix $\rmS$ is said to follow an EC matrix-variate  Wishart
distribution with DF  $n$, scale parameter $\Sigma$ and
CG $\varphi$, written as $\rmS\sim \ECW_m(n,\Sigma,\varphi)$, if there exists a random matrix  $\rmX\sim \EC_{m,n}(0,\Sigma,I_n,\varphi)$ such that $\rmS \overset{d}{=} \rmX\rmX^\top$.
\end{definition}
If $n>m$, then the PDF of $\rmS$ can be written as 
\begin{equation}
f_{\rmS}(\sfS)=
\dfrac{\pi^{mn/2}}{\Gamma_m(n/2)|\Sigma|^{n/2}}|\sfS|^{(n-m-1)/2}g(\tr(\Sigma^{-1}\sfS)),
\end{equation}
where $g(\cdot)$ is the density generator of $\rmX$. For $n<m$, we have the
singular matrix-variate EC Wishart distribution. For completeness, we derive the PDF of the functionally independent elements of $\rmS$  when $n<m$ in  Section \ref{sec:singularecwishart}.
 We now define the EC TV Wishart distribution. % that is
                                % the tensor-variate generalization of
                                % the matrix-variate case studied in~\citet{srivastavaandkhatri79,srivastava03}.
%We now define the EC tensor-variate Wishart distribution. %using the canonical matricization of \eqref{canonical}.
\begin{definition}\label{def:tenswish}
The random tensor 
%$\rtS \in\mathbb{R}^{\times_{k=1}^pm_k\times\times_{k=1}^pm_k}$ 
$\rtS \in\mathbb{R}^{\times_{j=1}^p m_j}%1\times m_2\times\dots\times
                                %m_p\times   m_1\times m_2\times
                                %\dots\times m_p}
$ 
 follows a tensor-valued
EC Wishart distribution with DF $n$, scale matrices
$\Sigma_1,\Sigma_2,\sdots,\Sigma_p$ and CG $\varphi$ ({\em i.e.},
$\rtS\sim
\ECW_{\bbm}(n,\Sigma_1,\sdots,\newline\Sigma_p,\varphi)$)
if $\rtS_{<p>}\sim \ECW_{m}(n,\Sigma,\varphi)$. 
\end{definition}
In the vector-variate case, the Wishart distribution can be
constructed from the vector outer product sum of independent and identically distributed (IID) MVN-distributed
random vectors. Similarly, the EC tensor-variate Wishart distribution can be constructed from the outer tensor product sum of uncorrelated tensors $\rtY_1,\rtY_2,\sdots,\rtY_n$ (where $\rtY_i = \rtY\times_{p+1}{\be_i^n}^\top$ for all $i=1,2,\dots,n$ and $\be_i^n \in \mbR^n$ is a unit basis vector with 1 as the $i$th
element and 0 elsewhere) which jointly follow
\begin{equation}\label{eq:jointfull}
\rtY\sim\EC_{[\bbm,n]^\top} (\mM_n, \sigma^2\Sigma_1,\Sigma_2, \sdots, \Sigma_p,I_n,\varphi).
\end{equation}
Here $\Sigma_k$ is constrained to have $\Sigma_k(1,1) = 1$ for all $k=1,2,\dots,p$ while $\sigma^2$ captures the overall proportionality constraint of $\Sigma$, and 
 $\mM_{n}\times_{p+1}{\be_i^n}^\top = \mM$ for all $i=1,2,\sdots,n$.
 In the next theorem, we show that $\rtY_1 ,\rtY_2,\sdots\rtY_n$ are uncorrelated, have identical marginal distributions,  and that their tensor outer product sum follows the EC Wishart distribution.
\begin{theorem}\label{thm:tenswish1}
Let $ \rtY_1, \rtY_2\hdots, \rtY_n$ jointly follow the distribution in
\eqref{eq:jointfull}. Then, we have:
\begin{enumerate}
\item \label{thm:tenswish1:1}
 $\rtY_i\sim\EC_{\bbm} (\mM, \sigma^2\Sigma_1, \Sigma_2,\sdots, \Sigma_p,\varphi)$ and $\forall i\neq j, \mathbb{E}\left(\vecc(\rtY_i-\mM)\vecc(\rtY_j-\mM)^\top\right) = 0$.
\item \label{thm:tenswish1:2}
$
\sum\limits_{i=1}^n (\rtY_i \circ \rtY_i)
 \sim 
\ECW_{\bbm}(n,\sigma^2\Sigma_1,\Sigma_2,\sdots,\Sigma_p,\varphi).
$%\vspace*{-.2cm}
\end{enumerate}
Here $\circ$ denotes the tensor outer product that we define in Section \ref{app:tensdef}.
\end{theorem}
\begin{proof}
See the Supplementary Material Section \ref{proof:tenswish1}.
\end{proof}
In Section \ref{sec:uncorrML} we derive maximum likelihood estimators (MLEs)
estimators for $(\mM,\sigma^2,\newline\Sigma_1,\Sigma_2,\sdots,\Sigma_p)$
under the  assumption that $\rtY_1,\rtY_2,\sdots,\rtY_n$ are
uncorrelated, as implied in  \eqref{eq:jointfull}, which is a
generalization of the traditional IID assumption.
 Setting $\varphi(z) = \exp(-z/2)$ leads to 
the case where IID $\rtY_i\sim\N_{\bbm}(0,\sigma^2\Sigma_1,\Sigma_2,\sdots,\Sigma_p)$ results in $\sum_{i=1}^n (\rtY_i \circ \rtY_i) \sim \mW_{\bbm}(n,\sigma^2\Sigma_1,\Sigma_2,\sdots,\Sigma_p)$. 
 



